Towards More Accurate US Presidential Election via Multi-step Reasoning with Large Language Models

Can Large Language Models (LLMs) accurately predict election outcomes? While LLMs have demonstrated impressive performance in various domains, including healthcare, legal analysis, and creative tasks, their ability to forecast elections remains unknown. Election prediction poses unique challenges, such as limited voter-level data, rapidly changing political landscapes, and the need to model complex human behavior. To address these challenges, we introduce a multi-step reasoning framework designed for political analysis. Our approach is validated on real-world data from the American National Election Studies (ANES) 2016 and 2020, as well as synthetic personas generated by the leading machine learning framework, offering scalable datasets for voter behavior modeling. To capture temporal dynamics, we incorporate candidates' policy positions and biographical details, ensuring that the model adapts to evolving political contexts. Drawing on Chain of Thought prompting, our multi-step reasoning pipeline systematically integrates demographic, ideological, and time-dependent factors, enhancing the model's predictive power.

==> 04exp.tex <==
% \section{\underline{Validation} of the Pipelines and \underline{Prediction} for the 2024 US Election}
% \section{Prediction for the 2024 US Election}


% \subsection{Experiment Settings}

% -- I will update a new map later -- waiting for last four states--

\section{Prediction for the 2024 US Election}
\label{Prediction}

\subsection{Experiment Settings} 

We extend our multi-step reasoning pipeline to predict the outcome of the 2024 US Presidential Election, featuring Donald Trump and Kamala Harris as the primary candidates, which thus introduce differences from the 2020 results.
Same as in the 2020 simulations, we incorporate only the candidates' policy positions and backgrounds as time-sensitive inputs, excluding real-time data from social media or news sources to maintain consistency and control within the model’s input space.
We follow the same simulation setup used in \S \ref{subsec:evaluation_results}, utilizing identical hardware and LLM APIs. 
Since GPT-4o’s training corpus extends only until October 2023, this experiment evaluates the model’s ability to make predictions on future, unseen data. After the election, these predictions can be compared with the actual results, offering a unique opportunity to assess the LLM’s predictive capabilities.


Consistent with our prior methods, we simulate individual votes cast exclusively for the Democratic and Republican parties, omitting No-Preference votes from the analysis. The preference for Trump (Republican Party) in each state is calculated using Eq. (\ref{eq:prob}).
% \[
% \text{Probability} = \frac{\text{Republican Votes}}{\text{Republican Votes} + \text{Democratic Votes}}
% \]
We applied the V3 pipeline to all 50 states. As in previous experiments, we employed random sampling with proportional extraction of synthetic personas for each state, ensuring statistical significance while optimizing computational efficiency.
This state-level analysis tests the adaptability of our multi-step pipeline to unseen election data and provides a scalable framework for forecasting election outcomes with synthetic personas.


% One interesting part of this paper is that we used our multi-step reasoning pipeline—combined with 2024 time-dependent election information between Donald Trump and Kamala Harris to conduct an Election prediction. Similar to the 2020 approach, we included only the two parties' policy positions and candidates' background information as time-dependent inputs for the LLM, without incorporating other real-time information from social media or news reports. 

% Since GPT-4o’s training corpus only extends up to October 2023, the 2024 prediction tests the model's performance on unseen data. In the future, we can also compare these predictions with the actual election results, providing a unique evaluation of the LLM’s capabilities in generation and prediction tasks.

% Consistent with the methods described earlier, we focused solely on simulating individual votes cast for the Democratic and Republican parties, excluding No-Preference votes from the analysis. To maintain uniformity throughout the paper, we continued to use the following formula to calculate each state’s preference for the two candidates as  a preference towards Trump (Republican party) as: 

% $\text{Probability} = \frac{\text{Republican Votes}}{\text{Republican Votes} + \text{Democratic Votes}}$

% We applied the V3 pipeline to 49 states to obtain a broader prediction sample and better evaluate the LLM's ability to generate outcomes on unseen data, excluding only Rhode Island (RI) and Connecticut (CT) -- due to missing data. Same as in the previous approach, we employed random sampling with proportional extraction of synthetic personas for each state, ensuring statistical significance while optimizing computational efficiency. 


% \subsection{Prediction Results}

% Different with the 2020 prediction, the LLM’s forecast suggests that Trump will win Wisconsin (WI) in the 2024 election. Additionally, Trump’s support is projected to increase in swing and tipping point states such as Pennsylvania (PA), Michigan (MI), and New Hampshire (NH) compared to 2020, although he is still expected to lose these states by narrow margins.

% For the remaining states, the LLM predicts that Trump will win Arizona (AZ) but lose North Carolina (NC)—consistent with the 2020 prediction, despite the fact that the outcome was incorrect in the 2020 election. For the other swing states, as well as the deep red and blue states, the LLM’s predictions remain aligned with the 2020 forecasts, showing only minor fluctuations in vote shares. The detailed prediction results are presented in Figure~\ref{fig:2024prediction}.

% It is important to note that the current pipeline for 2024 prediction only incorporates the synthetic persona's demographic information, the 2024 policy positions of both parties, and the candidates' personal details. It does not account for other exogenous variables, such as public opinion or external shocks, which could potentially influence the election outcome. Therefore, the primary objective of this paper is not to achieve perfectly accurate predictions but to explore the LLM’s ability to generalize on unseen corpus and assess how closely these generalizations align with real-world outcomes.

% \subsection{Prediction Results}

% Unlike the 2020 prediction, the LLM's 2024 forecast suggests a shift in Wisconsin (WI), with Trump projected to win the state. Also, Trump’s support is expected to increase in other swing and tipping-point states, including Pennsylvania (PA), Michigan (MI), and New Hampshire (NH), compared to 2020. However, despite these gains, he is still forecasted to lose these states by narrow margins.

% In other key states, the LLM predicts that Trump will secure Arizona (AZ) but lose North Carolina (NC), consistent with the 2020 forecast, despite the incorrect outcome in the actual 2020 election. For the rest of the swing states, as well as the deep red and blue states, the predictions largely align with those from 2020, showing only minor variations in vote shares. Detailed results are presented in Figure~\ref{fig:2024prediction}.

\subsection{Prediction Results}

The LLM’s 2024 forecast reveals notable shifts from the 2020 election. A key change is in Wisconsin (WI), where Trump is now projected to win with 54.90\% of the vote, marking a significant shift. Trump also shows gains in other swing states, including Pennsylvania (PA) with 47.85\%, Michigan (MI) with 48.87\%, and New Hampshire (NH) with 46.39\%, though he is still forecasted to narrowly lose these states to Harris.

In other battlegrounds, Trump is predicted to carry Arizona (AZ) with 51.09\%, flipping it back to the Republicans, but lose North Carolina (NC) with 45.69\%—consistent with the 2020 forecast, despite the incorrect outcome in that election. As shown in Figure~\ref{fig:2024prediction}, Trump is expected to secure Florida (FL) with 53.62\% and Texas (TX) with 56.36\%, further strengthening his position. However, Harris holds an edge in Nevada (NV) with 34.77\%, Georgia (GA) with 44.36\%, and Minnesota (MN) with 44.23\%. These results indicate highly competitive dynamics in key swing states, where narrow margins could determine the final outcome.

In other traditional red and blue states, Trump retains strong support in red states such as Arkansas (AR) with 69.69\% and Alabama (AL) with 67.20\%. Meanwhile, Harris is projected to maintain dominance in Democratic strongholds like California (CA) with 19.18\%, New York (NY) with 22.41\%, and Illinois (IL) with 30.36\%. Notably, in Alaska (AK)—a state that has remained red for the past 52 years—the LLM predicts a narrow Democratic victory with 49.39\% of the vote in 2024. It is worth mentioning that our preliminary test of the LLM on the 2020 Alaska election yielded an accurate Republican win with 52.42\%, making the predicted 2024 shift even more intriguing, as it could subtly tip the scales toward the Democrats.


Based on the LLM’s predictions and the winner-takes-all electoral vote allocation, Harris (Democratic Party) is projected to narrowly defeat Trump (Republican Party) with 270 (267 + 3 in Washington, D.C.) electoral votes to Trump’s 268. Trump’s strength in major Republican states like Texas and Florida underscores his resilience, while Harris’s performance in strongholds such as California and New York reaffirms Democratic dominance.
The tight margins in swing states like Pennsylvania, Georgia, and Arizona emphasize how slight shifts in voter preferences can still alter the outcome, demonstrating the fine balance between the two.

% The 2024 forecast by the LLM reveals several notable shifts compared to the 2020 prediction. 
% A key change is in Wisconsin (WI), where Trump is now projected to win with 54.90\% of the vote, marking a significant shift from 2020. Additionally, Trump shows improved performance in other swing and tipping-point states, including Pennsylvania (PA) with 47.85\%, Michigan (MI) with 48.87\%, and New Hampshire (NH) with 46.39\%. However, despite these gains, he is still forecasted to narrowly lose these states to Harris.

% For other critical states, the LLM predicts Trump will carry Arizona (AZ) with 51.09\% of the vote, flipping it back to the Republicans, but lose North Carolina (NC) with 45.69\%, consistent with the 2020 forecast despite the incorrect actual result in that election. In deep red states such as Texas (TX) with 56.36\% and Alabama (AL) with 67.20\%, Trump retains strong support. 
% Similarly, Kamala Harris is expected to maintain dominance in traditional Democratic strongholds like California (CA) with 19.18\%, New York (NY) with 22.41\%, and Illinois (IL) with 30.36\%.

% The overall results indicate competitive dynamics in key swing states, where narrow margins may determine the final outcome. As shown in Figure~\ref{fig:2024prediction}, Trump is projected to win several battleground states like Georgia (GA) and Florida (FL) with 44.36\% and 53.62\%, respectively, strengthening his position. However, Harris still holds the edge in certain critical regions like Nevada (NV) with 34.77\%. 

% Based on the LLM’s predictions and the winner-takes-all electoral vote allocation, Kamala Harris (Democratic Party) is projected to secure a narrow victory over Donald Trump (Republican Party) with 270 electoral votes to Trump’s 268. Trump’s strong performance in key states like Texas, Florida, and Ohio highlights his dominance in traditionally Republican regions. Meanwhile, Harris is expected to perform well in Democratic strongholds such as California, New York, and Illinois. 

% The inclusion of previously excluded states—Connecticut (CT) and Rhode Island (RI)—using their 2020 results brings Harris’s total to 270 electoral votes, solidifying her narrow win. The results emphasize the competitive dynamics in swing states like Pennsylvania, Georgia, and Arizona, where minor shifts in voter preferences could significantly alter the outcome. 

% \noindent
% \textbf{Prediction Results}.
% Based on the LLM’s predictions and the winner-takes-all electoral vote allocation, Trump is projected to win 268 electoral votes compared to Harris’s 259, securing a narrow victory. 
% However, if we were to include the excluded states—Connecticut (CT) and Rhode Island (RI)—using their 2020 results, Harris's total would rise to 270 electoral votes, resulting in a razor-thin margin in favor of the Democratic candidate.

% \noindent
% \textbf{Prediction Results}.  




% \noindent
% \textbf{Limitations}.
% It is important to note that the 2024 prediction pipeline relies solely on synthetic persona demographics, the policy positions of both parties, and the candidates' biographical information. It does not factor in external variables, such as shifts in public opinion or unexpected events, which could significantly influence the election outcome.
% As such, the objective of this paper is not to provide definitive predictions but to assess the LLM’s capacity to generalize on unseen data and to explore how well these generalizations align with real-world results. This experimental approach offers a novel lens for evaluating the model's predictive abilities and adaptability in dynamic political environments.

\noindent
\textbf{Limitations}.
The 2024 prediction pipeline relies on synthetic persona demographics, party policy positions, and candidate biographical information. While this controlled framework ensures consistency, it introduces certain limitations.
\textit{First}, the model does not account for shifts in public opinion, media narratives, or unexpected events—such as economic shocks or political scandals—that could alter voter behavior.
\textit{Second}, the simulation assumes static demographics from 2020 to 2024, neglecting any population shifts or migration patterns, even if small, that could affect state-level outcomes.

Note that \textit{this paper's objective is not to provide definitive forecasts but rather to showcase the potential of LLMs to generalize on unseen data}. This experimental setup highlights how well these models align with real-world patterns, serving as a demonstration of their predictive capacity rather than a source of fully reliable election predictions. 







% \section{Discussion and Future Directions (we may combine these into Section 4 if necessary)}

% observations

% limitations
% For 2024 Prediction we didn't capture any timely information from social media and candidates' recent performance on debates and election campaign

% potential of LLMs:
% - adversarial: agenda design
